A Comprehensive Low and High-level Feature Analysis for Early Rumor Detection on Twitter

Recent work have done a good job in modeling rumors and detecting them over microblog streams. However, the performance of their automatic approaches are not relatively high when looking early in the diffusion. A first intuition is that, at early stage, most of the aggregated rumor features (e.g., propagation features) are not mature and distinctive enough. The objective of rumor debunking in microblogs, however, are to detect these misinformation as early as possible. In this work, we leverage neural models in learning the hidden representations of individual rumor-related tweets at the very beginning of a rumor. Our extensive experiments show that the resulting signal improves our classification performance over time, significantly within the first 10 hours. To deepen the understanding of these low and high-level features in contributing to the model performance over time, we conduct an extensive study on a wide range of high impact rumor features for the 48 hours range. The end model that engages these features are shown to be competitive, reaches over 90% accuracy and out-performs strong baselines in our carefully cured dataset.

==> acknowledgement.tex <==

\vspace{0.25cm}
\noindent\textbf{Acknowledgements.} {This work was funded by the 
%EU FP7 project ForgetIT (Grant No. 600826)\footnote{\url{http://www.forgetit-project.eu/}}. % and the 
ERC Advanced Grant ALEXANDRIA (under the grant No. 339233).
}


==> dataset-websci17.tex <==
\section{Data Collection}
\label{sec:prep}



==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}


==> relatedwork-websci17.tex <==
\vspace{-0.2cm}
\section{Related Work}
\label{sec:rw}

A variety of issues have been investigated using data, structural information, and the dynamics of the microblogging 
platform Twitter including event detection \cite{kimmey2015twitter}, spam detection ~\cite{ahmed2012mcl,wang2010don}, or sentiment detection~\cite{barbosa2010robust}. Work on rumor detection in Twitter is 
less deeply researched so far, although rumors and their 
spreading have already been investigated for a long time in psychology ~\cite{allport1947psychology,borge2012absence,sunstein2014rumors}.
%People research on Twitter for a long time and there are a lots directions  to study this complex social network like event detection \cite{kimmey2015twitter}, spam detection ~\cite{ahmed2012mcl,wang2010don}, or sentiment detection~\cite{barbosa2010robust}. 
%~\cite{} use the structure of different communication networks including Twitter to identify the influential spreaders of rumor events.  
For Twitter, researcher first began from studying rumor spreading for special types of events such as natural disasters~\cite{mendoza2010twitter,tanaka2012transmission}, or terrorist attacks \cite{starbird2014rumors}. Tanaka et al.~\cite{tanaka2012transmission}, for example, analyze how psychological factors influence the information transmission via tweets. %But these results are not general enough to other types of rumors. 
Castillo et al. researched the information credibility on Twitter\cite{castillo2011information,gupta2014tweetcred}. The work, however, is based solely on people's attitude (trustful or not) to a tweet, not the credibility of the tweet itself. In other words, a false rumor tweet can be trusted by a reader, but it might anyway contain false information. The work still provides a good start of researching rumor detection. The work is further extended in \cite{liu2015real,yang2012automatic}, where different feature sets are used. Yang et al.~\cite{yang2012automatic}, e.g., added the location of the poster and the client type of user (web client or mobile phone) as additional important features.

Due to the importance of information propagation for rumors and their detection, there are also different simulation studies~\cite{seo2012identifying,tripathy2010study} about rumor propagations on Twitter. Those works provide relevant insights, but such simulations cannot fully reflect the complexity of real networks. Furthermore, there are recent work on propagation modeling based on epidemiological methods~\cite{bao2013new,jin2013epidemiological,kwon2013prominent}, yet over a long studied time, hence how the propagation patterns perform at early stage is unclear. Recently, ~\cite{wu2015false} use unique features of Sina Weibo to study the propagation patterns and achieve good results. Unfortunately Twitter does not give such details of the propagation process as Weibo, so these work cannot be fully applied to Twitter. 
%Furthermore, there is recent rumor detection research based on the propagation structure of rumors on Sina Weibo (a microblog platform in China)~\cite{wu2015false}. This work uses unique features of Sina Weibo to study the propagation pattern of rumors and achieve good results. Unfortunately Twitter doesn't give such details of the propagation process as Weibo, so these work cannot be fully applied to Twitter.
%In addition, this work focuses on only one kind of rumors, ``the false photos'' on social networks. 

Most relevant for our work is the work presented in~\cite{ma2015detect}, where a time series model to capture the time-based variation of social-content features is used. We build upon the idea of their \textit{Series-Time Structure}, when building our approach for early rumor detection with our extended dataset, and we provide a deep analysis on the wide range of features change during diffusion time
%Eunsoo et al.~\cite{seo2012identifying} build a simulation system with random sources of rumors using propagation graphs to detect the sources.
%To exploit the temporal dynamics,  use a time series model to capture the time-based variation of social-content features. We use their Series-Time Structure with our extended dataset and we provide a deep analysis on the wide range of features change during diffusion time. 


%Xiaomo et al. claimed their system is the first real time rumor debunking system on Twitter \cite{liu2015real}. But their work are similar with above other previous works, they use the static features of rumors and ignored the feature's changing over time during the event developing on the social network, but one feature called "crowd wisdom" is an new idea and we use it in our work.

%Other work use propagation models like SpikeM~\cite{kwon2013prominent}, SEIZ~\cite{jin2013epidemiological} to capture the changing of tweets' volume over time. These features are effective yet fail to fully produce effects in the early stage of rumor spreading as we further show later Section~\ref{featureanalyzing}. Bao et al. used SPNR model which is an extended SIS model as a strategy to control rumors \cite{bao2013new}. 

%J Ma et al. used Recurrent Neural Networks for rumor detection \cite{madetecting}, they input the tweet of rumor event into RNN time sequentially. Without any other handcrafted features, they got almost 90\% accuracy. As the same disadvantage of all kinds of Neural Networks models, the process of training model is a black box to us, so we cannot know the reason why we got this result. In our case, we cannot get the evidences to convince people why the detected event is more likely to be a rumor or rather than a breaking news. 
